Memory Based Online Learning of Deep Representations from Video Streams

We present a novel online unsupervised method for face identity learning from video streams. The method exploits deep face descriptors together with a memory based learning mechanism that takes advantage of the temporal coherence of visual data. Specifically, we introduce a discriminative feature matching solution based on Reverse Nearest Neighbour and a feature forgetting strategy that detect redundant features and discard them appropriately while time progresses. It is shown that the proposed learning procedure is asymptotically stable and can be effectively used in relevant applications like multiple face identification and tracking from unconstrained video streams. Experimental results show that the proposed method achieves comparable results in the task of multiple face tracking and better performance in face identification with offline approaches exploiting future information. Code will be publicly available.

==> ablative.tex <==
\begin{table*}[h]
	\centering
	\caption{Ablative study on using temporal coherence in ID tracking and on using a second pass without deleting the memory (2nd-pass).}
	\label{table-compare-gt}
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ Apink }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                130 &              69.3 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                265 &              74.9 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                107 &              65.8 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                178 &              72.9 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ BrunoMars }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                391 &              75.8 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                741 &              81.8 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                310 &              76.8 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                557 &              82.9 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ Darling }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                361 &              68.7 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                655 &              72.0 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                319 &              75.7 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                571 &              78.8 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ GirlsAloud }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                469 &              67.6 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                897 &              70.6 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                367 &              68.5 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                648 &              71.3 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ HelloBubble }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                160 &              83.4 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                295 &              87.5 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                149 &              85.3 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                253 &              89.5 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ PussycatDolls }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                316 &              64.9 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                884 &              67.3 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                306 &              62.4 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                865 &              64.6 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ Tara }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                542 &              60.4 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &               1025 &              62.4 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                483 &              59.2 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                768 &              61.3 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|}
				\hline
				\multicolumn{5}{|c|}{\textsc{ Westlife }}\\
				\hline
				Method                 & Mode    &   IDS $\downarrow$ &   MOTA $\uparrow$ &   MOTP $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt     & \bf{Online}  &                138 &              86.2 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & \bf{Online}  &                274 &              87.9 &             100.0 \\
				\textbf{MuFTiR}-gt     & 2nd-pass &                139 &              86.9 &             100.0 \\
				\textbf{MuFTiR}-gt-nc  & 2nd-pass &                240 &              88.5 &             100.0 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
\end{table*}

==> fp-bbt.tex <==

\begin{table}[h]
    \centering
    \caption{The three components of error in MOTA using ground truth as detector or a real face detector on Big Bang Theory}
    \label{table:ids-fp-fn-bbt}
        
\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e01 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &   FN &    FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                218 & 1361 &     0 &              96.0 \\
 \textbf{MuFTiR}-tiny & Online &                 24 & 4917 & 10787 &              59.9 \\
\hline
\end{tabular}}
\end{minipage}%
\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e02 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &   FN &    FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                178 & 3947 &     0 &              86.3 \\
 \textbf{MuFTiR}-tiny & Online &                 57 & 5598 & 10885 &              45.1 \\
\hline
\end{tabular}}
\end{minipage}\par\medskip

\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e03 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &   FN &    FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                191 & 6999 &     0 &              79.6 \\
 \textbf{MuFTiR}-tiny & Online &                 14 & 10857 &  8992 &              43.6 \\
\hline
\end{tabular}}
\end{minipage}%
\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e04 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &    FN &   FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                341 &  2345 &    0 &              92.1 \\
 \textbf{MuFTiR}-tiny & Online &                 84 &  8888 & 7015 &              53.2 \\
\hline
\end{tabular}}
\end{minipage}\par\medskip

\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e05 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &   FN &    FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                381 & 3130 &     0 &              89.8 \\
 \textbf{MuFTiR}-tiny & Online &                 36 & 10021 &  8981 &              44.5 \\
\hline
\end{tabular}}
\end{minipage}%
\begin{minipage}{.4\linewidth}\centering
    \resizebox{1\textwidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\textsc{ bbt\_s01e06 }}\\
\hline
 Method               & Mode   &   IDS $\downarrow$ &    FN &    FP &   MOTA $\uparrow$ \\
\hline
 \textbf{MuFTiR}-gt   & Online &                559 &  5449 &     0 &              87.4 \\
 \textbf{MuFTiR}-tiny & Online &                222 & 15990 & 11054 &              42.9 \\
\hline
\end{tabular}}
\end{minipage}\par\medskip

\end{table}

==> fp-poi.tex <==

\begin{table*}[h]
	\centering
	\caption{The three components of error in MOTA using ground truth as detector or a real face detector on Music Dataset}
	\label{table:ids-fp-fn-poi}
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ Apink }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                130 & 2105 &    0 &              69.3 \\
				\textbf{MuFTiR}-tiny & Online &                191 & 2627 &  446 &              55.1 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ BrunoMars }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                391 & 3644 &    0 &              75.8 \\
				\textbf{MuFTiR}-tiny & Online &                420 & 4178 & 3950 &              48.8 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ Darling }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                361 & 2620 &    0 &              68.7 \\
				\textbf{MuFTiR}-tiny & Online &                449 & 2278 &  887 &              62.1 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ GirlsAloud }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                469 & 4837 &    0 &              67.6 \\
				\textbf{MuFTiR}-tiny & Online &                339 & 6691 & 1272 &              49.3 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ HelloBubble }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                160 &  707 &    0 &              83.4 \\
				\textbf{MuFTiR}-tiny & Online &                 88 & 2150 &  301 &              51.4 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ PussycatDolls }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                316 & 4697 &    0 &              64.9 \\
				\textbf{MuFTiR}-tiny & Online &                 83 & 7050 & 2764 &              30.7 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ Tara }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                542 & 5210 &    0 &              60.4 \\
				\textbf{MuFTiR}-tiny & Online &                270 & 8259 &  259 &              39.5 \\
				\hline
		\end{tabular}}
	\end{minipage}%
	\begin{minipage}{.4\linewidth}\centering
		\resizebox{1\textwidth}{!}{
			\begin{tabular}{|l|l|r|r|r|r|}
				\hline
				\multicolumn{6}{|c|}{\textsc{ Westlife }}\\
				\hline
				Method               & Mode   &   IDS $\downarrow$ &   FN &   FP &   MOTA $\uparrow$ \\
				\hline
				\textbf{MuFTiR}-gt   & Online &                138 & 1433 &    0 &              86.2 \\
				\textbf{MuFTiR}-tiny & Online &                 76 & 3403 & 1198 &              58.9 \\
				\hline
		\end{tabular}}
	\end{minipage}\par\medskip
	
\end{table*}
